Elastic-dLLM: Position Preserving Context Compression and Augmentation of Diffusion LLMs

Unlike autoregressive models, which generate one token at a time, dLLMs denoise a chunk of [MASK] tokens jointly and sample one or more tokens per step; despite enabling parallel decoding, this process incurs substantial computational cost due to the large chunk size of masked tokens. We observe that much of this cost is spent on repeatedly processing the preceding context and many [MASK] tokens with the same feature representations, indicating considerable computational redundancy. In this work, we revisit dLLM's redundancy from the perspective of [MASK] tokens. Through systematic analysis, we verify the redundancy of [MASK] tokens while revealing their critical role in providing structural information. Guided by these findings, we propose position-preserving [MASK] token compression and terminal-aware augmentation. By compressing redundant [MASK] computation, this approach accelerates decoding and further provides a natural extension toward context-folding-like long-context scaling under limited input-length constraints for full-sequence dLLMs such as LLaDA-8B-Instruct and LLaDA-1.5. Moreover, for block dLLMs such as LLaDA2.0-mini, it augments the context with a protected terminal [MASK] token to enhance generation quality with negligible overhead.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction state that Elastic-dLLM provides training-free position-preserving context compression, iterative folding for long generation, and terminal-aware context augmentation for block dLLMs. The supporting observations are presented in \S\ref{sec:observation}, the method in \S\ref{sec:method}, and the benchmark results in \S\ref{sec:experiments}.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: \S\ref{sec:conclusion} discusses the scope of the method, including its focus on diffusion LLM decoding.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper proposes a training-free inference method and does not make formal theorem-style claims.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose the information needed to reproduce the main experimental results?
    \item[] Answer: \answerYes{}
    \item[] Justification: \S\ref{sec:setup} specifies models, datasets, decoding settings, generation length, temperature, hardware, and evaluation protocols. Appendix~\ref{app:impl} further states the compact layout, RoPE handling, sample counts, and percentage rounding convention.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to reproduce the main experimental results?
    \item[] Answer: \answerNo{}
    \item[] Justification: Code is not included in this submission. The evaluated benchmarks and model families are publicly documented and cited, and the method is specified sufficiently for re-implementation.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all training and test details necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Elastic-dLLM is training-free. \S\ref{sec:setup} reports the inference settings for full-sequence and block dLLMs, including denoising steps, block size, maximum generation length, temperature, terminal anchor setting, and hardware.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars or other appropriate information about statistical significance?
    \item[] Answer: \answerNo{}
    \item[] Justification: The reported benchmark accuracies are deterministic 0-shot evaluations under fixed decoding settings. The paper reports exact evaluation set sizes in Appendix~\ref{app:impl}; repeated-seed variance is not applicable to temperature-0 decoding.

\item {\bf Experiments compute resources}
    \item[] Question: Does the paper provide sufficient information on compute resources needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: \S\ref{sec:setup} states that experiments run on NVIDIA RTX 3090 GPUs and gives the relevant decoding configuration. The method is an inference-time context modification and does not require additional training compute.

\item {\bf Code of ethics}
    \item[] Question: Does the research conform with the NeurIPS Code of Ethics?
    \item[] Answer: \answerYes{}
    \item[] Justification: The work studies inference efficiency for language diffusion models using public benchmarks. It does not involve human subjects, private data, or new high-risk data collection.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss potential positive and negative societal impacts?
    \item[] Answer: \answerYes{}
    \item[] Justification: \S\ref{sec:conclusion} discusses efficiency benefits and limitations. The method reduces inference cost for existing dLLMs and does not introduce new model capabilities beyond those of the underlying models.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards for responsible release of high-risk assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper introduces an inference-time algorithm, not a new dataset or model checkpoint.

\item {\bf Licenses for existing assets}
    \item[] Question: Are creators or original owners of assets properly credited and are licenses and terms respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: The models, baselines, and benchmarks used in the evaluation are cited in \S\ref{sec:setup} and Table~\ref{tab:full_seq_main}. Users should follow the respective licenses and terms for the underlying models and datasets.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented?
    \item[] Answer: \answerNA{}
    \item[] Justification: No new dataset or model weights are introduced. The proposed inference procedure is documented in \S\ref{sec:method} and Appendix~\ref{app:impl}.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing or human-subject experiments, does the paper include instructions, screenshots, and compensation details?
    \item[] Answer: \answerNA{}
    \item[] Justification: No crowdsourcing or human-subject study is involved.

\item {\bf Institutional review board approvals}
    \item[] Question: Does the paper describe risks and IRB approvals for human-subject research?
    \item[] Answer: \answerNA{}
    \item[] Justification: No human-subject research is involved.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe LLM usage if it is an important, original, or non-standard component of the core method?
    \item[] Answer: \answerNA{}
    \item[] Justification: LLMs are the subject of evaluation, but no LLM is used as a non-standard component of the proposed method.

\end{enumerate}

